The Instinctive Bias: Spurious Images lead to Illusion in MLLMs

Large language models (LLMs) have recently experienced remarkable progress, where the advent of multi-modal large language models (MLLMs) has endowed LLMs with visual capabilities, leading to impressive performances in various multi-modal tasks. However, those powerful MLLMs such as GPT-4V still fail spectacularly when presented with certain image and text inputs. In this paper, we identify a typical class of inputs that baffles MLLMs, which consist of images that are highly relevant but inconsistent with answers, causing MLLMs to suffer from visual illusion. To quantify the effect, we propose CorrelationQA, the first benchmark that assesses the visual illusion level given spurious images. This benchmark contains 7,308 text-image pairs across 13 categories. Based on the proposed CorrelationQA, we conduct a thorough analysis on 9 mainstream MLLMs, illustrating that they universally suffer from this instinctive bias to varying degrees. We hope that our curated benchmark and evaluation results aid in better assessments of the MLLMs' robustness in the presence of misleading images. The code and datasets are available at https://github.com/MasaiahHan/CorrelationQA.

==> sections/append_arxiv.tex <==
\appendix


\begin{table*}[ht]{
\footnotesize
\centering
\resizebox{\textwidth}{!}{%}
% \tabcolsep2pt
\begin{tabular}{c|ccccccccccccc|c}
\toprule[1pt]
% Image & CogVLM & Idefics & IB. & M-gpt4. & mPLUG. & Qwen. & L-7B. & L-13B. & GPT4v \\
% \midrule
% Animal & 0.48 & 0.25 & 0.33 & 0.10 & 0.28 & 0.15 & 0.62 & 0.63} & 0.51\\
% Art & 0.70 & 0.76 & 0.73 & 0.34 & 0.61 & 0.62 & 0.78 & 0.78 &0.82} \\
% Color & 0.42 & 0.08 & 0.27 & 0.03 & 0.26 & 0.09 & 0.58} & 0.52 &0.15 \\
% City & 0.26 & 0.34 & 0.31 & 0.13 & 0.31 & 0.23 & 0.40 & 0.37 &0.41} \\
% Food & 0.35 & 0.28 & 0.28 & 0.08 & 0.21 & 0.22 & 0.39 & 0.46 & 0.50}\\
% History & 0 & 0.38 & 0.76 & 0.31 & 0.70 & 0.59 & 0.77 & 0.80} & 0.76\\
% Material & 0.32 & 0.16 & 0.25 & 0.05 & 0.27 & 0.21 & 0.42 & 0.43} &0.40 \\
% Natural & 0.57 & 0.51 & 0.53 & 0.20 & 0.46 & 0.42 & 0.58 & 0.61 & 0.70}\\
% Objects & 0 & 0.44 & 0.45 & 0.16 & 0.37 & 0.28 & 0.62 & 0.65} &0.51 \\
% Plant & 0.21 & 0.17 & 0.15 & 0.06 & 0.15 & 0.09 & 0.35 & 0.39} &0.26 \\
% Sports & 0.61 & 0.51 & 0.59 & 0.21 & 0.53 & 0.40 & 0.71 & 0.73 & 0.74}\\
% Technology & 0 & 0.62 & 0.72 & 0.23 & 0.73 & 0.64 & 0.80 & 0.82} & 0.76\\
% \midrule
% Average & 0.32 & 0.38 & 0.45 & 0.16 & 0.41 & 0.33 & 0.59 & 0.60} &0.55 \\
 Image& Animal & Art & Color & City & Food & History&Human & Material & Natural & Objects & Plant & Sports &Tech. & Average \\
\midrule
CogVLM & 0.48 & \cellcolor{lightblue}\textbf{0.70} & 0.42 & 0.26 & 0.35 & 0 &\cellcolor{lightblue}0.70& 0.32 & 0.57 & 0 & 0.21 & 0.61 & \cellcolor{lightblue}0 & 0.36 \\
Idefics & 0.25 &\cellcolor{lightblue} 0.76 & 0.08 & 0.34 & 0.28 & 0.38 &\cellcolor{lightblue}\textbf{0.83}& 0.16 & 0.51 & 0.44 & 0.17 & 0.51 & \cellcolor{lightblue}0.62 & 0.41 \\
InstructBlip & 0.33 &\cellcolor{lightblue} 0.73 & 0.27 & 0.31 & 0.28 &0.76&\cellcolor{lightblue}\textbf{0.82} & 0.25 & 0.53 & 0.45 & 0.15 & 0.59 & \cellcolor{lightblue}0.72 & 0.48 \\
MiniGPT-4 & 0.10 &\cellcolor{lightblue}0.34 & 0.03 & 0.13 & 0.08 & 0.31 &\cellcolor{lightblue}\textbf{0.50}& 0.05 & 0.20 & 0.16 & 0.06 & 0.21 &\cellcolor{lightblue} 0.23 & 0.19 \\
mPLUG-Owl2 & 0.28 & \cellcolor{lightblue}0.61 & 0.26 & 0.31 & 0.21 & 0.70 &\cellcolor{lightblue}\textbf{0.77}& 0.27 & 0.46 & 0.37 & 0.15 & 0.53 &\cellcolor{lightblue}0.73 & 0.44 \\
Qwen-VL & 0.15 &\cellcolor{lightblue} 0.62 & 0.09 & 0.23 & 0.22 &0.59 &\cellcolor{lightblue}\textbf{0.70}& 0.21 & 0.42 & 0.28 & 0.09 & 0.40 & \cellcolor{lightblue}0.64 & 0.36 \\
LLaVA-7B & 0.62 & \cellcolor{lightblue}0.78 & 0.58 & 0.40 & 0.39 & 0.77 &\cellcolor{lightblue}\textbf{0.88}& 0.42 & 0.58 & 0.62 & 0.35 & 0.71 &\cellcolor{lightblue} 0.80 & 0.61 \\
LLaVA-13B & 0.63 &\cellcolor{lightblue} 0.78 & 0.52 & 0.37 & 0.46 &0.80&\cellcolor{lightblue}\textbf{0.92} & 0.43 & 0.61 & 0.65 & 0.39 & 0.73 &\cellcolor{lightblue} 0.82 & 0.62 \\
GPT-4V & 0.51 & \cellcolor{lightblue}\textbf{0.82} & 0.15 & 0.41 & 0.50 &0.76 &\cellcolor{lightblue} 0.80& 0.40 & 0.70 & 0.51 & 0.26 & 0.74 &\cellcolor{lightblue} 0.76 & 0.57 \\
\midrule
Average &0.37&\cellcolor{lightblue}0.68&0.27&0.31&0.31&0.56&\cellcolor{lightblue}\textbf{0.77}&0.28&0.51&0.39&0.20&0.56&\cellcolor{lightblue}0.59& 0.45\\

\bottomrule[1pt]
\end{tabular}
}}
\caption{Accuracy (Acc) of MLLMs on \benchname{} under twelve categories when applied spurious image. We highlight the top three accuracy categories in blue background. \textbf{Bold} values are the maximum accuracy for each model.  }
\label{dataset3}
\end{table*}

\vspace{1.5cm}

\begin{table*}[ht]{
\footnotesize
\centering
\resizebox{\textwidth}{!}{%}
\begin{tabular}{c|ccccccccccccc|c}
\toprule[1pt]
% Typography  & CogVLM & Idefics & IB. & M-gpt4. & mPLUG. & Qwen. & L-7B. & L-13B.  \\
% \midrule
% Animal & 0.34 & 0.19 & 0.23 & 0.18 & 0.18 & 0.12 & 0.54 & 0.60}  \\
% Art   & 0.53  & 0.48 & 0.32 & 0.34 & 0.30 & 0.25 & 0.73} & 0.56  \\
% Color & 0.32 & 0.03 & 0.28 & 0.09 & 0.12 & 0.07 & 0.59} & 0.43  \\
% City & 0.06 & 0.03 & 0.04 & 0.03 & 0 & 0.03 & 0.38} & 0.32 \\
% Food & 0.29 & 0.14 & 0.15 & 0.05 & 0.09 & 0.13 & 0.38 & 0.47}  \\
% History &0 & 0.41 & 0.48 & 0.26 & 0.37 & 0.22 & 0.76} & 0.71 \\
% Material & 0.09 & 0.04 & 0.10 & 0.02 & 0.08 & 0.04 & 0.42 & 0.53} \\
% Natural & 0.46 & 0.33 & 0.35 & 0.17 & 0.27 & 0.24 & 0.59 &0.61}  \\
% Objects &0 & 0.36 & 0.22 & 0.20 & 0.22 & 0.14 & 0.57 & 0.67}  \\
% Plant & 0.11 & 0.09 & 0.08 & 0.06 & 0.05 & 0.03 & 0.26 & 0.40} \\
% Sports &0.53 & 0.38 & 0.40 & 0.14 & 0.30 & 0.27 & 0.73 & 0.75}  \\
% Technology &0 & 0.17& 0.22 & 0.18 & 0.25 & 0.25 & 0.78 & 0.80}  \\
% % & 0.17 & 0.22 & 0.12 & 0.13 & 0.20 & 0.23 & \\
% \midrule
% Average &0.23 &0.22 &0.24 &0.14 &0.19 &0.15 &0.56 &0.57}\\
Typography & Animal &Art & Color & City & Food & History &Human& Material & Natural & Objects & Plant & Sports & Tech. & Average \\
\midrule
CogVLM & 0.34 &\cellcolor{lightblue} \textbf{0.53} & 0.32 & 0.06 & 0.29 & \cellcolor{lightblue}0 &0 & 0.09 & 0.46 & 0 & 0.11 &\cellcolor{lightblue}\textbf{ 0.53} & 0 & 0.21 \\
Idefics & 0.19 &\cellcolor{lightblue} \textbf{0.48}& 0.03 & 0.03 & 0.14 & \cellcolor{lightblue}0.41&0.40 & 0.04 & 0.33 & 0.36 & 0.09 & \cellcolor{lightblue}0.38 & 0.17 & 0.23 \\
InstructBlip & 0.23 &\cellcolor{lightblue} 0.32 & 0.28 & 0.04 & 0.15 & \cellcolor{lightblue}0.48 &\textbf{0.56} & 0.10 & 0.35 & 0.22 & 0.08 & \cellcolor{lightblue}0.40 & 0.22 & 0.26 \\
MiniGPT-4 & 0.18 & \cellcolor{lightblue}0.34 & 0.09 & 0.03 & 0.05 & \cellcolor{lightblue}0.26 &\textbf{0.44} & 0.02 & 0.17 & 0.20 & 0.06 & \cellcolor{lightblue}0.14 & 0.18 & 0.16 \\
mPLUG-Owl2 & 0.18 & \cellcolor{lightblue}0.30 & 0.12 & 0 & 0.09 &\cellcolor{lightblue} \textbf{0.37}&0.31 & 0.08 & 0.27 & 0.22 & 0.05 & \cellcolor{lightblue}0.30 & 0.25 & 0.20 \\
Qwen-VL & 0.12 & \cellcolor{lightblue}0.25 & 0.07 & 0.03 & 0.13 &\cellcolor{lightblue} 0.22 &0.19 & 0.04 & 0.24 & 0.14 & 0.03 &\cellcolor{lightblue} \textbf{0.27 }& 0.25 & 0.15 \\
LLaVA-7B & 0.54 &\cellcolor{lightblue} 0.73 & 0.59 & 0.38 & 0.38 &\cellcolor{lightblue} 0.76 &0.49 & 0.42 & 0.59 & 0.57 & 0.26 &\cellcolor{lightblue}0.73 & \textbf{0.78} & 0.55 \\
LLaVA-13B & 0.60 &\cellcolor{lightblue} 0.56 & 0.43 & 0.32 & 0.47 &\cellcolor{lightblue} 0.71 &0.37 & 0.53 & 0.61 & 0.67 & 0.40 &\cellcolor{lightblue} 0.75 & \textbf{0.80} & 0.54 \\
GPT-4V & 0.70 &\cellcolor{lightblue} 0.57 & 0.19 & 0.39 & 0.58 &\cellcolor{lightblue} \textbf{0.86}&0.84 & 0.38 & 0.67 & 0.72 & 0.39 &\cellcolor{lightblue} 0.79 & 0.36 & 0.57 \\
\midrule
Average &0.34&\cellcolor{lightblue}0.45&0.23&0.14&0.27&\cellcolor{lightblue}0.45 &0.40&0.19&0.41&0.35&0.17&\cellcolor{lightblue}\textbf{0.48}&0.33&0.32 \\
\bottomrule[1pt]
\end{tabular}
}}
\caption{Accuracy (Acc) of MLLMs on \benchname{} under twelve categories when applied spurious typography. We highlight the top three accuracy categories in blue background. \textbf{Bold} values are the maximum accuracy for each model.}
\label{dataset4}
\end{table*}

\section{Detailed Prompts Example}
\label{sec:appendix}
\begin{figure*}
    \centering
    \includegraphics[width=0.8\textwidth]{image_and_pdf/append.pdf}
    \caption{Prompt template and examples of QA pairs creation using GPT-4.}
    \label{appendix}
\end{figure*}

\autoref{appendix} displays an example of generating question-answer (QA) pairs with GPT-4.  We detail the system prompt for the animal category and provide three example QA pairs for GPT-4 as references. Due to the output token limit, GPT-4 could only produce 10 QA pairs once, so we require it to continue generating more examples.

\section{More Experiments}
\subsection{Manual Verification}
 We randomly sample 20\% of the QA pairs from each category and verify if the actual answers match the true answers provided by GPT-4. The authenticity rates for QA pairs in each category are displayed in \autoref{manual}. Most of the categories have higher than 90\% authenticity rates except the class city. The reason is that in the city category, there are some fictional cities from the movies and novels besides the real world, which results in naming conflict.




\subsection{Accuracy Results on Spurious Image}
\label{append2}
In \autoref{dataset3} and \autoref{dataset4}, we present the accuracy of 9 MLLMs on spurious natural image and spurious typography, respectively. 

For the spurious natural image, categories like art, human, technology and history reach higher accuracy, which aligns with our analysis in \autoref{qualitative}. For categories such as art, technology and history, the spurious answers are often non-visualizable concepts (e.g., 5G technology, the Battle of Waterloo), and in the human category, spurious image containing portraits or photographs are unrecognizable to MLLMs, thus failing to significantly deceive or mislead the models.




For the spurious typography, accuracy across all 13 categories is more uniform. Compared to natural image, the application of typography results in a lower average accuracy for each category. We assume that since the content of typography solely consists of OCR text which does not involve understanding the content and is independent of the category, MLLMs are more directly misled by spurious information. 

\begin{table}[H]
\centering
\footnotesize
\begin{tabular}{M{0.3\columnwidth}|M{0.25\columnwidth}|M{0.25\columnwidth}}
\toprule[1pt]
Class      & Questions & Authenticity rate  \\ 
\midrule
Animal     &  105  & 100\%      \\
Art        &    105&  100\%     \\
City      &    90&  78\%      \\
Color       &   99&     95\%      \\
Food       & 100  &    95\%      \\
History    & 105   &    100\%     \\
Material   &  90  &    90\%     \\
Natural    &   100 &    100\%      \\
Objects    &   105 &    100\%   \\
Plant      &  105  &    91\%    \\
Sports     & 95  &     95\%     \\
Technology &   105 &    100\%       \\ 
\midrule
Average      &  101&     97\%     \\
\bottomrule[1pt]
\end{tabular}

\caption{We present the total number of questions and the Authenticity rate of \benchname. We randomly sample 20\% of QA pairs from each category and manually verify the Authenticity of true answers given by GPT-4. }
\label{manual}
\end{table}

\subsection{Accuracy Declined Ratio}
We additionally defined \textbf{Accuracy declined ratio} to identify which categories experience the largest proportion of accuracy decline in MLLMs. The definition of accuracy declined ratio is as follows:
\begin{gather}
    ADR=\frac{AccDrop}{Acc_{f}},
\end{gather}
where $AccDrop$ denotes the pre-defined Accuracy drop metric of MLLMs, and $Acc_{f}$ represents accuracy on factual image. A higher accuracy declined ratio indicates more severely affected by spurious information, which is similar to AccDrop but emphasizes the relative effects.

\autoref{dataset5} and \autoref{dataset6} display the accuracy declined ratio results for natural image and typography. 
Our findings are consistent with those in \autoref{append2}. For natural image, categories like animal, color, and plant which consist of tangible entities experience a higher accuracy decline ratio. With typography, the accuracy decline ratio for all categories exceeds 30\%. After applying spurious images, the decline ratio for typography in every category is higher than for natural images.

\begin{table*}[ht]
\footnotesize
\centering
\resizebox{\textwidth}{!}{%}
\begin{tabular}{c|ccccccccccccc|c}
\toprule[1pt]

Image \textcolor{red}{$\downarrow$} & Animal & Art &Color  & City & Food & History &Human& Material & Natural & Objects & Plant & Sports & Tech. & Average \\
\midrule
% CogVLM&0.45&0.08&0.49&0.41&0.46&0.0&0.2&0.5&0.12&0.0&0.71&0.19&0.0&0.35\\
% Idefics&0.67&0.01&0.33&0.26&0.54&-0.03&0.06&0.61&0.2&0.37&0.69&0.32&0.11&0.31\\
% InstructBlip&0.62&0.04&0.66&0.33&0.55&0.08&0.04&0.59&0.16&0.44&0.78&0.28&0.09&0.35\\
% MiniGPT-4&0.82&0.21&0.73&0.41&0.8&0.09&0.04&0.79&0.0&0.71&0.86&0.6&0.23&0.49\\
% mPLUG-Owl2&0.65&0.1&0.69&0.3&0.55&0.01&0.06&0.49&0.21&0.52&0.74&0.33&0.06&0.35\\
% Qwen-VL&0.76&0.13&0.83&0.48&0.68&0.03&0.18&0.68&0.28&0.58&0.86&0.49&0.06&0.45\\
% LLaVA-7B&0.03&0.02&0.13&-0.03&0.02&0.01&0.02&0.11&-0.02&0.03&0.13&0.05&0.0&0.03\\
% LLaVA-13B&0.05&0.0&0.16&0.12&0.06&0.0&-0.01&0.14&0.05&0.07&0.17&0.08&0.02&0.07\\
% GPT-4V&0.45&0.15&0.83&0.27&0.42&0.14&0.12&0.5&0.2&0.43&0.68&0.21&0.17&0.36\\
CogVLM&\cellcolor{lightblue}45\%&8\%&\cellcolor{lightblue}49\%&41\%&46\%&0\%&20\%&50\%&12\%&0\%&\cellcolor{lightblue}\textbf{71\%}&19\%&0\%&35\%\\
Idefics&\cellcolor{lightblue}67\%&1\%&\cellcolor{lightblue}33\%&26\%&54\%&-3\%&6\%&61\%&20\%&37\%&\cellcolor{lightblue}\textbf{69\%}&32\%&11\%&31\%\\
InstructBlip&\cellcolor{lightblue}62\%&4\%&\cellcolor{lightblue}66\%&33\%&55\%&8\%&4\%&59\%&16\%&44\%&\cellcolor{lightblue}\textbf{78\%}&28\%&9\%&35\%\\
MiniGPT-4&\cellcolor{lightblue}82\%&21\%&\cellcolor{lightblue}73\%&41\%&80\%&9\%&4\%&79\%&0\%&71\%&\cellcolor{lightblue}\textbf{86\%}&60\%&23\%&49\%\\
mPLUG-Owl2&\cellcolor{lightblue}65\%&10\%&\cellcolor{lightblue}69\%&30\%&55\%&1\%&6\%&49\%&21\%&52\%&\cellcolor{lightblue}\textbf{74\%}&33\%&6\%&35\%\\
Qwen-VL&\cellcolor{lightblue}76\%&13\%&\cellcolor{lightblue}83\%&48\%&68\%&3\%&18\%&68\%&28\%&57\%&\cellcolor{lightblue}\textbf{86\%}&49\%&6\%&45\%\\
LLaVA-7B&\cellcolor{lightblue}3\%&2\%&\cellcolor{lightblue}\textbf{13\%}&-3\%&2\%&1\%&2\%&11\%&-2\%&3\%&\cellcolor{lightblue}\textbf{13}\%&5\%&0\%&3\%\\
LLaVA-13B&\cellcolor{lightblue}5\%&0\%&\cellcolor{lightblue}16\%&12\%&6\%&0\%&-1\%&14\%&5\%&7\%&\cellcolor{lightblue}\textbf{17\%}&8\%&2\%&7\%\\
GPT-4V&\cellcolor{lightblue}45\%&15\%&\cellcolor{lightblue}\textbf{83\%}&27\%&42\%&14\%&12\%&50\%&20\%&43\%&\cellcolor{lightblue}68\%&21\%&17\%&36\%\\
\midrule
Average &\cellcolor{lightblue}50\%&8\%&\cellcolor{lightblue}53\%&28\%&45\%&3\%&7\%&49\%&13\%&35\%&\cellcolor{lightblue}\textbf{62}\%&28\%&8\%&30\% \\

\bottomrule[1pt]
\end{tabular}
}
\caption{Accuracy declined ratio (the ratio between AccDrop (AccDrop) and Accuracy (Acc) on factual image) in natural image. It reflects the proportion of accuracy decline when models are exposed to spurious image compared to factual ones. We highlight the top three accuracy categories in blue background. \textbf{Bold} values are the maximum AccDrop proportion for each model.}
\label{dataset5}
\end{table*}




\begin{table*}[!h]
\footnotesize
\centering
\resizebox{\textwidth}{!}{%}
\begin{tabular}{c|ccccccccccccc|c}
\toprule[1pt]

Typography \textcolor{red}{$\downarrow$} & Animal & Art & Color & City & Food &History &Human& Material & Natural & Objects & Plant & Sports & Tech. & Average \\
\midrule
CogVLM&65\%&45\%&67\%&\cellcolor{lightblue}\textbf{93\%}&67\%&0\%&0\%&\cellcolor{lightblue}91\%&49\%&0\%&\cellcolor{lightblue}88\%&45\%&0\%&69\%\\
Idefics&78\%&48\%&87\%&\cellcolor{lightblue}\textbf{96\%}&84\%&34\%&60\%&\cellcolor{lightblue}95\%&61\%&60\%&\cellcolor{lightblue}90\%&56\%&77\%&71\%\\
InstructBlip&76\%&60\%&71\%&\cellcolor{lightblue}\textbf{95\%}&83\%&42\%&40\%&\cellcolor{lightblue}89\%&62\%&77\%&\cellcolor{lightblue}91\%&59\%&77\%&72\%\\
MiniGPT-4&75\%&51\%&73\%&\cellcolor{lightblue}95\%&92\%&47\%&48\%&\cellcolor{lightblue}\textbf{97\%}&72\%&64\%&\cellcolor{lightblue}87\%&81\%&70\%&73\%\\
mPLUG-Owl2&82\%&65\%&88\%&\cellcolor{lightblue}\textbf{100\%}&90\%&61\%&68\%&\cellcolor{lightblue}91\%&66\%&76\%&\cellcolor{lightblue}94\%&68\%&74\%&78\%\\
Qwen-VL&87\%&72\%&93\%&\cellcolor{lightblue}97\%&86\%&71\%&80\%&\cellcolor{lightblue}96\%&73\%&84\%&\cellcolor{lightblue}\textbf{97\%}&71\%&69\%&83\%\\
LLaVA-7B&18\%&14\%&16\%&\cellcolor{lightblue}7\%&-6\%&4\%&\textbf{49\%}&\cellcolor{lightblue}19\%&2\%&12\%&\cellcolor{lightblue}45\%&5\%&4\%&17\%\\
LLaVA-13B&9\%&27\%&40\%&\cellcolor{lightblue}33\%&8\%&13\%&\textbf{60\%}&\cellcolor{lightblue}9\%&13\%&-8\%&\cellcolor{lightblue}25\%&4\%&2\%&21\%\\
GPT-4V&13\%&37\%&\textbf{79\%}&\cellcolor{lightblue}32\%&31\%&9\%&11\%&\cellcolor{lightblue}59\%&26\%&10\%&\cellcolor{lightblue}33\%&17\%&51\%&32\%\\
\midrule
Average&55\%&46\%&68\%&\cellcolor{lightblue}\textbf{72\%}&59\%&31\%&46\%&\cellcolor{lightblue}71\%&47\%&41\%&\cellcolor{lightblue}\textbf{72\%}&45\%&47\%&57\% \\

\bottomrule[1pt]
\end{tabular}
}
\caption{Accuracy declined ratio (the ratio between AccDrop (AccDrop) and Accuracy (Acc) on factual image) in typography. It reflects the proportion of accuracy decline when models are exposed to spurious image compared to factual ones. We highlight the top three accuracy categories in blue background. \textbf{Bold} values are the maximum AccDrop proportion for each model.}
\label{dataset6}
\end{table*}










==> sections/intro.tex <==
\section{Introduction} 
Large language models (LLMs) have sparked a transformative shift in the field of artificial intelligence~\cite{zhao2023survey, workshop2022bloom,chowdhery2023palm,touvron2023llama}. %significantly propelling technological advancements in the field of artificial intelligence. 
Following the development of LLMs, a series of multi-modal large language models (MLLMs) have emerged to enable LLMs with visual processing capabilities~\cite{alayrac2022flamingo,gong2023multimodal,yin2023survey,zhu2023minigpt}.
% \LQ{
% Large Language Models (LLMs) have sparked a transformative shift in the field of artificial intelligence \cite{zhao2023survey}, significantly propelling technological advancements. 
% Inspired by the success of LLMs, 
% Following the development of the technology, a series of Multi-modal Large Language Models (MLLMs) capable of supporting visual modality inputs and outputs have emerged by incorporating with LLMs \cite{alayrac2022flamingo,gong2023multimodal,yin2023survey,zhu2023minigpt}. Contemporary mainstream MLLMs typically employ pre-trained image encoders to extract visual features, using LLM as the text encoder. This approach involves training on visual-text pairs and projecting image features into the textual feature space to unify modalities, which releases great visual-semantic understanding for MLLMs. Furthermore, these models have demonstrated commendable performance in downstream tasks such as Visual Question-Answering(VQA) \cite{goyal2017making} and image captioning\cite{hodosh2013framing}.
% }
Typically, current MLLMs process visual inputs by converting them into visual tokens that share the same latent space as language tokens in LLMs. This conversion not only maintains excellent text processing abilities but also enables LLMs with powerful visual semantic understanding capabilities.
These models have demonstrated commendable performance in downstream tasks such as image captioning~\cite{hossain2019comprehensive, mplug} and visual question-answering~(VQA)~\cite{goyal2017making, pali}.
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{image_and_pdf/casenew.pdf}
    \caption{Cases of Instinctive Bias in LLaVA. \\
    \textbf{Top (Factual image)}: when presented with images that correspond to one of the correct answers (\textit{i.e.} Elon Musk), MLLMs can respond to the correct answer.\\
    \textbf{Middle (Spurious image)}: when presented with images that are related but do not correspond to the correct answer (\textit{i.e.} Steve Jobs), MLLMs are hallucinated to provide an incorrect answer.\\
    \textbf{Bottom (Text-only)}: without spurious images, MLLMs display the ability to provide the correct answer.}
    \label{examplecase}
    \vspace{-4mm}
\end{figure}

% Evaluation of MLLMs on our proposed benchmark \benchname. We apply accuracy to assess the hallucination rate. The higher accuracy indicates that MLLM answers correctly when accompanied with deceptive image conditions.
 
% However, some image inputs utilized by MLLMs might provide \replaced{spurious information that misleads MLLMs to produce more erroneous responses if those models rely excessively on the visual inputs}{misleading information thus leading to the increased likelihood of producing erroneous responses for MLLMs if they rely excessively on the visual inputs}. 
% Our research has been driven by the observation that MLLMs are more prone to providing \replaced{incorrect}{misleading} answers when accompanied by \replaced{instinctive but spurious}{misleading} images (correlated to the true answer but different) \deleted{after undergoing image-text alignment training}, while this hallucination\added{ phenomenon} does not occur in text-only QA scenarios with LLMs. 
% Some examples are shown in \autoref{examplecase}. 
% % Here we define the spurious images as those that can induce MLLMs hallucination from their content.
% \prj{Here, we define spurious images as those capable of inducing hallucinations in MLLMs due to their content.}
% Moreover, MLLMs yield high accuracy in responses to random and unrelated images.
% %significance
% \replaced{This finding is pivotal given the wide usage of MLLMs in real-world scenarios and the naturalness of those spurious images, where any human users might be asking the same type of questions. On top of that, hallucination under some certain category of scenarios, such colors, can lead to disastrous results, e.g. when MLLMs were equipped in automatic driving cars and misled by real-time visual inputs of traffic lights. To quantify the effect of those issues in modern MLLMs, a standard benchmark becomes necessary. }{This finding is pivotal as, firstly, human evaluators can discern the non-relevance of images to questions and respond correctly, and secondly, this issue has practical implications in real-world applications as MLLMs become more widely utilized.
% So it has led us to design a benchmark aimed at assessing the performance of MLLMs on this issue.}


% Despite the success achieved by state-of-the-art MLLMs on commonsense QA, the 


% Despite the success achieved by state-of-the-art MLLMs, they still suffer from different types and extent of hallucination. 
% \tyh{Existing research primarily focuses on hallucinations on the tasks where the image and answer are consistent, such as image description and image-based question-answering (QA). 
% However, there has been limited study on hallucinations from complex image-text reasoning, where images and answers are inconsistent. 
% We identify such hallucination as instinctive bias. 
% Typically, instinctive bias are common in scenarios like analogy recommendations, and image reasoning, especially when users face information gaps or hard-to-describe images.} 
% % \shizhe{why do users provide misleading information? should illustrate}
% \tyh{\autoref{examplecase} shows a specific example of instinctive bias. We first define spurious images as those having contents correlated to the question but different from the true answer. %, which are capable of inducing hallucinations in MLLMs. 
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{image_and_pdf/rader.pdf}
    \vspace{-8mm}
    \caption{Accuracy of MLLMs on natural spurious images in our proposed benchmark \benchname. The higher accuracy indicates that MLLMs answer correctly when accompanied by spurious images.}
    \label{rader}
    \vspace{-4mm}
\end{figure}


Despite the success achieved by state-of-the-art MLLMs, most studies mainly focus on simple visual-textual relationships, (\textit{i.e.} factual image: the image directly corresponds to the answer), such as image description and image-based question answering. However, it is still under-explored that if current models can handle complex visual-textual relationships (\textit{i.e.} spurious image: the image is related to the answer but does not directly correspond to them.). Typically, this kind of visual relationship is common in scenarios like analogy recommendations, and image reasoning, especially when users face information gaps or hard-to-describe images.
In \autoref{examplecase}, we show a specific example of MLLMs in handling different kinds of input images, where under the text-only condition and multi-modal condition with factual image, LLaVA can accurately respond the correct answer (\textit{i.e.} Elon Musk). However, when the image is only with Steve Jobs, LLaVA assumes Steve Jobs to be the corresponding answer and ignores the semantics of the question. This observation is crucial considering the widespread use of MLLMs in real-world scenarios, where spurious images resembling those that human users might encounter can lead to the same type of misleading questions. 
Therefore, it is essential to establish a benchmark to quantify the impact of such issues in current MLLMs.
\tyh{ssss}
% \LQ{
% Despite the success achieved by state-of-the-art MLLMs, most studies mainly focus on simple visual-textual relationships, (\textit{i.e.} factual image: the image and answer are consistent), such as image description and image-based question answering. However, it is still under-explored that current models can handle complex visual-textual relationships (\textit{i.e.} spurious image: the image and answer are related but inconsistent). Typically, this kind of visual relationship is common in scenarios like analogy recommendations, and image reasoning, especially when users face information gaps or hard-to-describe images.
% In \autoref{examplecase}, we show a specific example of MLLMs in handling different kinds of input images, where 
% }


% Our research has been motivated by the observation that MLLMs are particularly susceptible to provide incorrect answers when presented with instinctive yet spurious images. 
% Notably, we observe that this phenomenon does not occur in text-only question-answering scenarios with LLMs, nor when presenting the MLLMs with images that are unrelated to the question. 


% In this paper, we introduce a novel benchmark \added{called} \benchname{} to assess the degree of hallucination in MLLMs when spurious visual prompts are presented. 
% The constructed dataset contains commonsense QA pairs in 13 categories, which \added{consists of} over 7,000 questions-answers (QA) pairs with answer-related images to mislead MLLMs.
To study the hallucination of MLLMs under spurious visual inputs, we design a novel benchmark called \benchname{}. \benchname{} collects over 7,000 question-answer (QA) pairs in 13 categories, where each pair contains multiple answer-related images that may mislead MLLMs. Specifically, we first use GPT-4~\citep{2303.08774} to generate meaningful QA pairs with five related but incorrect answers and a correct one. Based on the generated answers, we leverage the advanced diffusion model to generate the corresponding spurious and factual images for each question.
In addition to natural images, we also generate five typographic images for spurious answers, inspired by \citet{mmsafety}. 
Based on the design benchmark, we conducted an in-depth analysis to uncover the instinctive bias present in mainstream MLLMs. 
Our findings, presented in \autoref{rader}, demonstrate that 9 state-of-the-art MLLMs including GPT-4V suffer from hallucination when presented with spurious visual inputs. % despite performing well with factual images. 
This phenomenon indicates that by providing information related to spurious answers, images can induce MLLMs to instinctively focus on the visual content, resulting in responses that are predominantly based on visual information without proper reasoning and thinking. This is similar to the cases of unconscious decision-making processes observed in human brains~\citep{kahneman2011thinking,booch2021thinking}.

Our contributions are summarized as follows:
\textbf{1)} We first identify the visual instinctive bias in MLLMs, where spurious visual inputs can cause current MLLMs to hallucinate.
% {We implement a pipeline capable of automatically creating intricate image-QA pairs crafted to hallucinate MLLMs.}
\textbf{2)} 
We propose \benchname{} to quantify the seriousness of instinctive bias across different types, demonstrating that this issue is universal across MLLMs.
% {We propose \benchname, a novel benchmark to assess the extent of hallucination of MLLMs when provided with different type of answer-related clues.}
\textbf{3)} We provide an in-depth analysis of the recent 9 representative MLLMs on our benchmark, showing their susceptibility to spurious visual inputs under different scenarios.


\begin{figure*}[t]
    \centering
    \includegraphics[width=1.06\textwidth]{image_and_pdf/frameworknew.pdf}
    \caption{Pipeline of our dataset construction. First, we utilize GPT-4 to generate a set of QA pairs with five spurious answers. Next, we leverage image generators to generate corresponding images based on these answers (natural and typography). Using these images, we construct a set of text and image pairs to evaluate the robustness of MLLMs to spurious images. 
    }
    \vspace{-3mm}
    \label{framework}
\end{figure*}
